EgoSonics: Generating Synchronized Audio for Silent Egocentric Videos

We introduce EgoSonics, a method to generate semantically meaningful and synchronized audio tracks conditioned on silent egocentric videos. Generating audio for silent egocentric videos could open new applications in virtual reality, assistive technologies, or for augmenting existing datasets. Existing work has been limited to domains like speech, music, or impact sounds and cannot capture the broad range of audio frequencies found in egocentric videos. EgoSonics addresses these limitations by building on the strengths of latent diffusion models for conditioned audio synthesis. We first encode and process paired audio-video data to make them suitable for generation. The encoded data is then used to train a model that can generate an audio track that captures the semantics of the input video. Our proposed SyncroNet builds on top of ControlNet to provide control signals that enables generation of temporally synchronized audio. Extensive evaluations and a comprehensive user study show that our model outperforms existing work in audio quality, and in our proposed synchronization evaluation method. Furthermore, we demonstrate downstream applications of our model in improving video summarization.

==> content/text/04_experiments.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=6.0in]{content/images/sync3.jpg} 
%\vspace{-10mm}
\caption{Figure compares how well each model can synchronize the generated audio with the GT audio. Our method can generate very synchronized audios with higher quality. On the other hand, Diff-Foley and Make-an-Audio fails to do so, and often fails to synthesize contextually correct audio. Diff-Foley can only synthesize 8 seconds long audio compared to 10 seconds for others.
% \ssinline{Is this supposed to be in experiments? Remove axis labels and make everything aligned.}
}
\label{fig:sync}
\end{figure*}

\section{Experiments}
\label{others}

\vspace{-3mm}
%

The goal of our experiments is to compare the audio and synchronization quality of generated audio, justify and ablate key design decisions, and demonstrate the application of our method in improving video summarization.
\vspace{-3mm}
\paragraph{Dataset.} 
%
We use one of the largest audio-visual egocentric datasets, Ego4D~\cite{ego4d}, which consists of roughly 3600 hours of egocentric videos capturing various daily activities.
However, not all videos in this dataset contain audio, and even those with audio do not always contain useful learnable information (e.g.,~background noise).
% And since, the dataset comprises of videos ranging from a few minutes to a few hours, not everything in the dataset is relevant for audio-visual activity correspondence.
% We noticed that sections of the video where the subject is performing some activity, have a significant presence of audio.
% For example, a person using drill machine to make a hole, a person washing dishes, or a person using sewing machine. 
Therefore, we focus on videos with useful learnable visual audio cues, and pick 10-second chunks as described in \Cref{subsec:avprep}.
% , where the RMS value of the audio exceeds a certain manually set threshold value.
After this process, we obtain around 150K videos with the corresponding audio.
% , which we use for training \shortname. 
We use STFT~\cite{perraudin2013fast} to convert these 10 seconds long audio waveform into spectrograms.
We sampled the audio at 22~KHz to get $E_A \in \mathbb{R} ^ {430 \times 1024}$.


\paragraph{Experimental Setup.} 

\begin{table*}[h]
\centering
%
\caption{\textit{V2A generation results comparing various methods over 3 metrics (FID, IS, VAAS). We have also compared them against the audio sampling rate, maximum frequency support, spectrogram size used, the length of generated audio, and the number of video frames used for guidance. Our method, using 30 fps, sampled at highest frequency can generate the highest resolution spectrogram for a 10 seconds long audio. It also outperforms the existing V2A on FID, IS, and VAAS.}}
%
\scalebox{0.95}{\begin{tabular}{c|c|c|c|c|c|c|c|c}
 \textbf{Method} &\textbf{ Audio SR} & \textbf{Max Freq.} & \textbf{Spec. Size} & \textbf{Audio Length} & \textbf{Video Frames} & \textbf{FID} $\downarrow$ & \textbf{IS} $\uparrow$ & \textbf{VAAS} $\uparrow$ \\
 \hline
 \hline
 Im2Wav & $16 KHz$ & $8 KHz$ & $-$ & $5 sec$ & $1-30fps$ & $91.73$ & $19.15$ & $59.24$ \\
 Make-an-Audio & $16 KHz$& $8 KHz$ & $80 \times 624$ & $9-10 sec$ & $1-4$ & $83.72$  &  $22.14$  & $64.57$ \\
 Diff-Foley & $16 KHz$ & $8 KHz$ & $256 \times 128$ & $8 sec$ & $4fps$ & $76.92$ & $37.92$ & $78.19$ \\
 \shortname (ours) & $22 KHz$ & $20 KHz$ & $512 \times 512$ & $10 sec$ & $30fps$ & $\textbf{41.14}$ & $\textbf{54.41}$ & $\textbf{92.77}$ 
%
\label{table:fid_compare} 
\end{tabular}}
%
\end{table*}
%
We train our model for 50 epochs on 8 Nvidia 3090 GPUs. 
Video embeddings and audio spectrograms are extracted from the 10-second clips and resized to 512$\times$ 512 to ensure synchronization between video and audio modalities.
We used the pretrained weights of CLIP Image encoder and used it to obtain $E_V$.
\modulename is initialized with the pretrained SD's UNet encoder weights, and the zero convolutions are initialized with zero weights to prevent issues in the generated results during initial iterations. 
We also use the same Classifier-Free Guidance Resolution Weighting scheme as proposed in \cite{controlnet}.

\begin{table}[ht]
% \vspace{-5mm}
\centering
%
\caption{\textit{Comparing the effect of using audio generated from different methods on improving video summarization task. It is interesting to note that, even the un-synchronized audios generated from our model have sufficient contextual information to outperform the existing methods.
% \ssinline{Table headers must be bold. Too much whitespace below the table. This seems like it could be a wrap figure. Or make the table wider.}
}}
% \vspace{0.2cm}
%
\scalebox{1.0}{\begin{tabular}{c|c}
 \textbf{Method} & \textbf{Cosine Similarity} $\uparrow$ \\
 \hline
 \hline
 Without Audio &  $0.67$ \\
 GT Audio &  $0.81$  \\
 \hline
 Im2Wav &  $0.57$  \\
 Make-an-Audio & $0.68$ \\
 Diff-Foley &  $0.71$  \\
 EgoSonics w/o Cross-Attn &  $0.72$ \\ 
 EgoSonics (ours) &  $\textbf{0.76}$
%
\label{table:vid_sum} 
\end{tabular}}
%
\end{table}
% \vspace{-3mm}
\paragraph{Metrics.}
%
For quantitative evaluation, we have used the two standard Frechet Distance (FID) and Inception Score (IS) as used in most previous works \cite{diff_foley, make_an_audio, sheffer2023hear}. FID is used to measure the distribution-level similarity with the dataset, IS is effective is measuring the sample quality and diversity. The proposed VAAS metrics is essential to measure how well the generated audio is synchronized with the video. Thus, it captures the alignment between the audio and video features.


\subsection{Qualitative and Quantitative Comparisons} 
%
Qualitative results generated from our pipeline are shown in \Cref{fig:results_1} (please also see supplementary video).
From the results, we see that our method not only generates good quality audio spectrograms corresponding to video activities but also achieves synchronization as depicted by the dotted lines where some distinct event in the video.
Moreover, we observe that our method implicitly learns to suppress background noise and only generate sounds of interest, thus acting as an \textbf{Implicit Noise Removal} technique.
This is the main reason why all the ground truth (GT) audios contain a lot of soft frequency components, but audio generated from our method does not. 
More results are presented in the supplementary.

% \subsection{Quantitative Results}
The quantitative results of our method are presented in Table~\ref{table:fid_compare}.
% \ssinline{Change to first person}
Our proposed method generating 10 seconds long audio with frequencies upto 20~KHz is able to generate better results than all the baselines in FID and IS measurement. Using 30 frames per second from the input video helped us in better alignment of the generated audio, thus, achieving a 14$\%$ increase in Video-Audio Alignment Score (VAAS).
% \ssinline{Say something about the VAAS metric here.}

\subsection{Video Summarization} 
%
To demonstrate applications of our method beyond just audio generation, we show that it can be used to improve the quality of video summarization. 
Video summarization \cite{video_summ} 
% involves providing a short summary of the video via understanding the video frames.
% \ssinline{Add citation to a video summarization paper that defines what summarization is.}
involves providing a short summary of a scene in a given video via understanding the video frames. 
We leverage the fact that audio provides additional cues about the scene~\cite{audio_video_floor1, audio_video_floor2} through the easily identifiable sounds associated with each activity.
Our aim is to incorporate the audio generated from our method alongside video encoding, and observe an improvement in the accuracy of video summarization. 
This will highlight the effectiveness of our method in generating relevant sounds capturing high-order details of the scene.
More details about the video summarization architecture are presented in the supplementary.
Table~\ref{table:vid_sum} compares the cosine similarity between the text embedding predicted from the video summarization model and the GT text embedding we generated using Ego4D narrations \cite{ego4d} for various methods.
It can be seen that the audio generated by EgoSonics can significantly help in predicting the correct text embedding and outperforms existing V2A methods.

\begin{table}[h]
% \vspace{-4mm}
\centering

\caption{\textit{Comparing the performance of our model against various changes, including removing the \textit{Syncronet} model, removing cross-attention in \textit{Syncronet}, and using video guidance at different fps.}
% \ssinline{Same comments as table 2.}
}
\vspace{0.2cm}

\scalebox{1.0}{\begin{tabular}{c|c|c}
 \textbf{Method} & \textbf{FID} & \textbf{VAAS} \\
 \hline
 \hline
 EgoSonics w/o Syncronet &  $150.28$  & $-$ \\
 EgoSonics w/o Cross-Attn & $\textbf{34.33}$ & $72.83$ \\
 EgoSonics $@4$ fps & $37.18$ & $84.97$ \\
 EgoSonics $@15$ fps & $40.72$ & $89.39$ \\
 EgoSonics $@30$ fps & $41.14$ & $\textbf{92.77}$

\label{table:ablation} 
\end{tabular}}

\end{table}

% \vspace{-3mm}
\subsection{Ablation Study}
% \vspace{2mm}

% \subsubsection{Analyzing Syncronet:}
\paragraph{w/o \modulename.}
%
Our method achieves better audio-visual synchronization since we use 30 frames per second to make \modulename learn the per-frame correspondences between audio and video. 
Here, we analyzed the effect of removing \modulename completely and solely using the mean video embedding to guide the Stable Diffusion. 
From the results, it can be seen that there is a significant drop in FID meaning the pre-trained Stable Diffusion cannot synthesize the good quality audio spectrograms. 
Consequently, SD is not able to generate conditional audio and lacks synchronization.

\vspace{-2mm}
\paragraph{w/o Cross-Attention in \modulename.}
%
Now, we also analyzed the effect of removing Cross-Attention with the video embedding $E_V$ in \modulename and just using Self-Attention as given in Eqn.~3.
% \ssinline{Where is equation 6? I cannot find it. PLease use CRef}
From \Cref{table:ablation}, it's clear that our method is able to synthesize good quality audio spectrograms as the FID score is good. However, the poor alignment score indicates that the local pixel level alignment control to achieve synchronization is coming from the control signals through cross-attention with the video embedding $E_V$ in the time domain.

\vspace{-2mm}
\paragraph{Effect of Video Rate on Alignment.}
%
Unlike previous methods that use an average video embedding, or 1-4~fps for conditioning the audio, we used 30~fps to extract the temporal information from the video for guidance.
In this section, we analyzed the impact of using 30 frames on AV synchronization.
We compared the performance of \modulename at different fps including 4~fps used by the current SOTA Diff-Foley \cite{diff_foley}.
From \Cref{table:ablation}, it can be seen that our method is not only able to generate good quality audio spectrograms, but also able to generate a VAAS score of 85.
However, as we increase the fps to 15, the alignment score increases to 89, and then to 92.77 with 30~fps. 


% \subsubsection{Stable Diffusion:}

% We also analyzed the impract of using Stable Diffusion $1.5$ vs $2.1$. 

==> macros.tex <==
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{multicol}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage{wrapfig}
\usepackage{changes}
\usepackage{xspace}
\usepackage{float}
\usepackage{amsmath}
\usepackage{cleveref}

\definechangesauthor[color=BrickRed]{SS}
\newcommand{\srinath}[2]{\added[id=SS,comment={\footnotesize#1}]{#2}}
\newcommand{\ssinline}[1]{\textcolor{red}{\textbf{Srinath}: #1}}

\newcommand{\Rone}{\textcolor{cb-salmon-pink}{\textbf{R1}\xspace}}
\newcommand{\Rtwo}{\textcolor{cb-green-sea}{\textbf{R2}\xspace}}
\newcommand{\Rthree}{\textcolor{cb-blue}{\textbf{R3}\xspace}}

\newcommand{\manu}{manu.\xspace}
\newcommand{\sm}{supp.\xspace}

\definecolor{cb-edit}     {RGB}{ 60, 170, 200}
\newcommand{\cbEdit}  [1]{\textcolor{cb-edit} {#1}}

\newcommand{\parahead}[1]{\noindent\textbf{#1}:\ }
\newcommand{\tabhead}[1]{\par\textbf{#1}}
% Packed itemize
\newenvironment{packed_itemize}
{\begin{itemize}
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
}{\end{itemize}}

\newenvironment{packed_enumerate}
{\begin{enumerate}
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newcommand{\filluptopage}[1]{%
  \clearpage
  \loop\ifnum\value{page}<#1\relax
    \null\clearpage
  \repeat
  \loop\ifnum\value{page}=#1\relax
    \null\clearpage
  \repeat
}

\makeatletter
\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother

\newcommand{\circlednumber}[1]{\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {#1}}}}
\newcommand{\circlednumberbold}[1]{\textbf{\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {#1}}}}}
